Memory-Induced Supra-Competitive Outcomes Between Deep Reinforcement Learning Agents in Optimal Trade Execution

In this paper, we investigate whether deep reinforcement-learning agents interacting in a shared optimal-execution environment can sustain supra-competitive outcomes, in the sense of achieving lower implementation shortfalls than the relevant game-theoretical competitive benchmark. We study a two-agent Almgren-Chriss liquidation game and examine how learned behavior depends on intra-episode environment feedback, the ability to interpret the mid-price and the agent's knoledge of the past. We first use ex-ante schedule-learning agents to remove intra-episode feedback and isolate what can arise when agents commit to complete liquidation trajectories before execution begins. We then allow agents to condition on the evolving state using a variety of DDQN architectures. We find that, when agents are given access to intra-episode history, especially recent prices and own past actions, supra-competitive outcomes become substantially more frequent and more persistent. These findings indicate that supra-competitive behavior in this execution game is driven not by multi-agent learning or by current price observation alone, but by feedback, memory, and state-contingent interaction along the realized execution path.

==> sections/next_steps.tex <==
\chapter{Future Work}
\label{sec:next_steps}

Several directions naturally follow from the present analysis. First, we plan to extend the study beyond the two-player case and investigate whether the qualitative patterns documented here persist in larger execution games. A particularly relevant comparison is between the symmetric two-player benchmark with initial inventories \((100,100)\) and a three-player game with inventories \((100,50,50)\), which preserves the same aggregate initial inventory but changes the strategic structure of the interaction. This will allow us to ask whether learning agents effectively infer the number of competitors in the market and adapt toward the corresponding Nash benchmark, or whether the richer interaction structure makes supra-competitive outcomes even more likely.

Second, we plan to study the extent to which supra-competitive outcomes survive \emph{out-of-sample}. In the current experiments, training and testing are performed in closely matched environments. An important next question is therefore whether policies that appear collusive in-sample continue to generate collusive-like behavior when evaluated in perturbed environments, for example under different initial inventories, horizons, impact coefficients, or volatility levels. Put differently, we would like to understand whether collusion-like behavior in these games is merely environment-specific, or whether it generalizes as a robust strategic pattern beyond the exact training configuration.
